Curriculum Offline Imitation Learning

Offline reinforcement learning (RL) tasks require the agent to learn from a pre-collected dataset with no further interactions with the environment. Despite the potential to surpass the behavioral policies, RL-based methods are generally impractical due to the training instability and bootstrapping the extrapolation errors, which always require careful hyperparameter tuning via online evaluation. In contrast, offline imitation learning (IL) has no such issues since it learns the policy directly without estimating the value function by bootstrapping. However, IL is usually limited in the capability of the behavioral policy and tends to learn a mediocre behavior from the dataset collected by the mixture of policies. In this paper, we aim to take advantage of IL but mitigate such a drawback. Observing that behavior cloning is able to imitate neighboring policies with less data, we propose \textit{Curriculum Offline Imitation Learning (COIL)}, which utilizes an experience picking strategy for imitating from adaptive neighboring policies with a higher return, and improves the current policy along curriculum stages. On continuous control benchmarks, we compare COIL against both imitation-based and RL-based methods, showing that it not only avoids just learning a mediocre behavior on mixed datasets but is also even competitive with state-of-the-art offline RL methods.

==> papers/checklist.tex <==
\clearpage
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYES{}
  \item Did you describe the limitations of your work?
    \answerYES{See \se{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYES{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYES{See \theo{thm:1} and \ap{ap:proof}.}
	\item Did you include complete proofs of all theoretical results?
    \answerYES{See \ap{ap:proof}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYES{See supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYES{See \se{se:exp1} and \se{se:hyperparameter}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYES{See \tb{tab:final} and \tb{tab:d4rl}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYES{We use the dataset from D4RL~\cite{fu2020d4rl} benchmark as said in \se{se:d4rl}}
  \item Did you mention the license of the assets?
    \answerNO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYES{We include our code and our dataset in the supplemental material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYES{We use a public dataset.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> papers/trash.tex <==
\section{Theoretical Analysis}
\label{sec:discussion}
\subsubsection{Sample Analysis for Behavior Cloning} The quantity-quality dilemma gives two necessary conditions for BC to learn a good policy: high-quality, and enough data. The first condition is quite clear that BC simply imitates the behavior policy, resulting in the limitation inherently. The second condition, intuitively makes sense due to the narrow support of the dataset provided by few samples. 
However, such requirements can be relaxed as shown in \se{sec:motivation}, where a policy closed to the demonstrated policy can still stably imitate the behavior policy by BC with limited demonstrations. 
Beyond such observations, we develop our theoretical analysis 
on how the number of samples affects the discrepancy between policies, with a slight assumption about the support of the policy.

\begin{assumption}
The data support of the behavior policy covers the whole state space $\caS$.
\end{assumption}
Under such an assumption we now present our bound:
% Considering real applications of reinforcement learning, this assumption is reasonable because a policy for the real environment needs to act properly under all possible circumstances in order to guarantee a minimal level of safety. Under this assumption, we propose \theo{th:1}.
\begin{theorem}[Limitation of direct BC]\label{th:1}
Given a training policy $\pi_e$, and a dataset $\caD$ collected by the behavior policy $\pi_b$, the empirical behavior policy derived from the dataset is $\hat{\pi}_b$. Suppose their occupancy measures are $\rho_e(s,a)$, $\hat{\rho}_b(s,a)$ and $\rho_b(s,a)$, and $\rho_*=\sup_{s,a} \rho_b(s,a)$. Then the total variation distance between $\rho_e(s,a)$ and $\rho_b(s,a)$ are bounded as:
\begin{equation}\label{eq:thm1}
    \TV(\rho_e(s,a)\|\rho_b(s,a)) \le \underbrace{ \TV(\rho_e(s)\|\hat{\rho}_b(s)) + \max_s\TV(\pi_e(a\mid s)\|\hat{\pi}_b(a\mid s))}_{\text{BC gap}} + \underbrace{O(\rho_*^{|\caD|})}_{\text{data gap}}
\end{equation}
\end{theorem}
\begin{proof}
See \ap{ap:proof}.
\end{proof}

This bound bridges $\pi_e$ and $\pi_b$ by the empirical behavior policy $\hat{\pi}_b$, splitting the discrepancy between the training policy and the behavior policy into two separated parts. The first part, BC gap, shows an upper bound of the intrinsic discrepancy that the training policy can learn from dataset only using BC. With theoretically enough times of update, the training policy can overfit onto the empirical behavior policy thus reducing the BC gap. The second part, which is much more important, is the data gap depending on the number of samples in the dataset, if the behavior policy is fixed. Since $\rho_*\leq 1$, the data gap will decay exponentially with respect to the number of samples.

Intuitively, this can also be explained by data support. If $\rho_*$ is close to $1$, i.e. $\rho_b(s,a)$ has a sharp peak, then samples drawn from this distribution will gather around the peak, resulting in a small data support, which suggests that the data gap will decay slowly as more samples are taken. On the contrary, a relatively flat $\rho_b(s,a)$ induces small $\rho_*$, from which sampling will generate rapidly expanding data support, thereby the data gap shrinks in the same manner.

